Distributional Robustness of Linear Contracts

Linear contracts are ubiquitous in practice, yet optimal contract theory often prescribes complex, nonlinear structures. We provide a distributional robustness justification for linear contracts. We study a principal-agent problem where the agent exerts costly effort across multiple tasks, generating a stochastic signal upon which the principal conditions payment. The principal faces distributional ambiguity: she knows the expected signal for each effort level, but not the full distribution. She seeks a contract maximizing her worst-case payoff over all distributions consistent with this partial knowledge. Our main result shows that linear contracts are optimal for such a principal. For any contract, there exists a linear contract achieving weakly higher worst-case payoff. The proof introduces the concavification approach built around the notion of self-inducing actions; these are actions where an affine contract simultaneously induces the action as optimal and supports the concave envelope of payments from above. We show that self-inducing actions always exist as maximizers of the gap between the concave envelope and agent's cost function. We extend these results to multi-party settings. In common agency with multiple principals, we show that affine contracts improve all principals' worst-case payoffs. In team production with multiple agents, we establish a complementary necessity result: if any agent's contract is non-affine, the unique ex-post robust equilibrium is zero effort. Finally, we show that homogeneous utility and cost functions yield tractable characterizations, enabling closed-form approximation ratios and a sharp boundary between computational tractability results.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}



\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper's main contribution and scope are summarized inthe abstract and introduction. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper has section discussing the limitations. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assumptions are clearly stated, and each for each theoretical result a complete proof is included. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Though this paper does not have large scale experiments, there are some numerical simulations that validate theoretical results. For the numerical simulations, enough details are provided for reproducibility. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: I currently did not release code. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Details are provided for the numerical experiments. 
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: I don't think this applies to the experiments in this paper. In particular, there is not a notion of ``mean" in the experiments. The experiments serve to show a quantity (the cumulative loss in an online learning problem) aligns with the upper bound in theoretical results. However, I did repeat the experiments multiple times. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The numerical experiments are ran on a personal laptop, which I also mentioned in the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The reesearch conform to the Code of Ethics. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: I discussed positive impacts and do not foresee negative impacts. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sec/abstract.tex <==
In this work, we study the multitasking principal-agent problem. The agent performs several task for the principal, and the principal posts a contract incentivizing the agent to exert effort. The principal can observe a signal for each task, and the contract is a mapping from the space of possible signals to a payment. We study the special class of linear contracts from three perspectives: robustness, uniformity, and learning. Firstly, we show a robustness result: in an ambiguous setting when only first moment information is known, there is a linear contract maximizing the principal's payoff in a worst-case scenario. Secondly, we show a uniformity result: when the agent's cost function is homogeneous to a certain degree and the the principal's utility takes a linear form across tasks, then the optimal contract depends on the agent's cost function only through its homogeneuity degree. Thirdly, we study the problem of learning an optimal linear contract through observational data. We identify this as an measurement error model, and propose instrumental regression methods to estimate the optimal contract parameters in an offline setting, or to learn the optimal contract in an online setting. 


==> sec/model.tex <==
% \section{The Model (OLD)}
% \szcomment{Since we changed focus to not only multitask, lets state in the general form. And mention in the multitask setting how would each parameter look like. }
% We study the principal-agent problem in which an agent exerts effort across $d$ dimensions, each representing a distinct task. The effort is denoted by $a\in \mathcal{A} \subset (\mathbb{R}^+)^d$, and we assume the cost function is strictly increasing, strictly convex, and twice differentiable on its domain with $c(0) = 0$. Each action generates a stochastic signal in the signal space denoted by $\mathcal{X} \subset (\mathbb{R}^+)^d$. The principal's contract is a mapping from the signal space $\mathcal{X}$ to a non-negative payment, so that the agent is protected by limited liability; we denote the contract by $w: \mathcal{X} \mapsto \mathbb{R}^+$. The agent's expected payment is then $\Ex_{x\sim F(a)} [w(x)]$, and his net utility is the expected payment minus cost:
% \[
% V_A(a) = \Ex_{x\sim F(a)}[w(x) | a] - c(a). 
% \]

% The agent's effort $a$ generates a gross utility for the principal, which we denote by $u(a): \mathcal{A} \mapsto \mathbb{R}^+$. The principal's surplus is the gross benefit minus the expected payment:
% \[
% V_P(a) = u(a) - \Ex_{x\sim F(a)}[w(x) | a]. 
% \]

% The timing of the interaction is as follows:
% \begin{enumerate}
% 	\item The principal offers a contract $w: \mathcal{X} \rightarrow \mathbb{R}^+$
% 	\item The agent chooses effort $a \in \mathcal{A}$ to maximize expected utility $V_A(a; w(\cdot))$, and incurs private cost $c(a)$
% 	\item The outcome $x \in \mathcal{X}$ is realized as $x\sim F(a)$
%     \item Payment $w(x)$ is transferred from principal to agent
% 	% \item The agent receives payment $w({x})$ 
% 	% \item The principal receives expected utility $u(a) - \ip{\phi}{a}$
% \end{enumerate}

% The signal space $\mathcal{X}$ may either be finite or infinite (continuous). For example, in the finite setting, each task may have binary outcomes $\mathcal{X} = \set{0,1}^d$. In the continous outcome setting, the signal space maybe the entire non-negative orthant $\mathcal{X} = (\bbR^+)^d$. We typically think of the agent's action space $\mathcal{A}$ as always being continuous. For example, in the multitask setting with binary outcomes for each task, we have $\mathcal{A} = [0,1]^d$, and the agent's action $a$ determines the (marginal) success probability for each task. In the continuous outcome setting we would then have $\mathcal{A} = \mathcal{X} = (\bbR^+)^d$. 

% % We first present the model and our main results for this binary outcome setting for expositional purpose; the extension to arbitrary finite outcome space is then trivial. We also discuss the extension to continuous outcome space. 

% \szcomment{Also revise this part. I think now binary outcome setting is like a spcieifc example we walkthrough in the multtask setting. Other than that, we just want to use this to demonstrate that unbiasedness is WLOG, and ease reviewers into this idea. }
% % \emph{Binary Outcome Setting. } We first focus on discrete case where outcomes are \emph{binary}: $\mathcal{X} = \set{0,1}^d$. In other words, each task has two possible outcomes: success or failure. In the binary outcome setting, the agent's action space $\mathcal{A} \coloneqq [0,1]^d$, where the $i$-th component $a_i$ represents the effort level on task $i$, and determines the \emph{success probability}. In other words we have that: 
% % \[
% % \Ex[x|a] = a. 
% % \]
% % All of our proof extend directly to the finite outcome setting. We obtain a slightly weaker characterization for robustness results in the continuous outcome setting, as we discuss in subsequent sections. 

% % The principal incentivizes the agent to exert effort through a contract. In general, a contract specifies a payment to the agent for each realized outcome, meaning that $2^d$ values must be specified:

% % \[
% % w: \set{0,1}^d \to \bbR^{+}. 
% % \]

% \paragraph{Linear and Affine Contracts. } A special class of contracts is that of \emph{linear contracts}, parameterized by $\phi \in (\mathbb{R}^+)^d$. Under a linear contract $\phi$, the agent receives a monetary transfer of $\langle \phi, x \rangle$ upon realization of outcome $x$. Another class is affine contracts, which are linear contracts with the addition of an offset term. Under the affine contract $\psi \in \mathbb{R}^{d+1}$, the payment to the agent (abusing notation using $\psi$ both as an operator and as a vector) is $\psi(x) = \psi_0 + \sum_{i\in[d]} \psi_i x_i$. 

% \subsection{Distributional Uncertainty and Robustness}

% Recall a contract is a mapping from outcomes to payments, denoted $w: \mathcal{X} \to \bbR^+$. We assume the agent is protected by limited liability, ensuring all payments are non-negative. Given a contract $w$ and a compatible family $\mathcal{F}$, let $a^*(w; \mathcal{F}) \in \arg\max_{a \in \mathcal{A}} \Ex_{x \sim F_a}[w(x)] - c(a)$ denote the agent's best response. The principal's expected utility is then
% \[
% V_P(w; \mathcal{F}) = u(a^*(w; \mathcal{F})) - \Ex_{x \sim F_{a^*(w; \mathcal{F})}}[w(x)].
% \]

% The principal's worst-case payoff from contract $w$ is defined as
% \begin{align}
% V_P(w) = \min_{\mathcal{F} \text{ compatible}} u(w; \mathcal{F}). \label{eq:robustnessObj}
% \end{align}


% We are interested in the setting where distribution only mean is known. \szcomment{Make sure reviewer understand unbiasedness is WLOG, maybe use the binary case as intro to ease them into the idea. } The principal is ambiguity averse, meaning he is optimizing
% \[
% xxx
% \]


\section{Multitasking Principal-Agent Problem}
\label{sec:problem-statement}
In this section we describe a basic setup of a bilateral principal-agent problem with a single principal and single agent. The two parties enters a contractual relation. The agent's effort (or action) space is $\mathcal{A}$. When he takes action $a \in \mathcal{A}$, he incurs a private cost $c(a)$. We usually assume the cost function $c: \mathcal{A} \to \mathbb{R}^+$ is strictly increasing, strictly convex, and twice differentiable on its domain, with $c(0) = 0$. The agent's effort generates a stochastic signal $x \in \mathcal{X}$, observable by both parties. We denote $F(a)$ as the mapping from the action space $\cA$ to a distribution over the signal space $\mathcal{X}$. In the multitask principal-agent setting we have $\mathcal{A}, \mathcal{X} \subset (\mathbb{R}^+)^d$, here $d$ represents the number of tasks, and for an effort vector $a\in\mathcal{A}$, the $i$-component $a_i$ is interpretated as the effort in the $i$-th task, and $x_i$ is interpretated as the signal for the $i$-th task. 

The principal offers a contract $w: \mathcal{X} \to \mathbb{R}^+$, specifying a non-negative payment for each realized signal. The non-negativity constraint reflects limited liability protection for the agent. Given a contract $w(\cdot)$ and the distribution mapping $F(\cdot)$ from actions to the signal space, the agent's expected utility is
\[
V_A(a; w(\cdot), F(\cdot)) = \Ex_{x \sim F(a)}[w(x)] - c(a),
\]
The agent takes an action maximizing his surplus:
\[
a^*(w(\cdot), F(\cdot)) \in \arg\max_a V_A(a; w(\cdot), F(\cdot)). 
\]
We assume ties are broken in favor for the principal. We may simply write $a^*$ when $w$ and $F$ are clear from context. 

Denote $u: \mathcal{A} \to \mathbb{R}^+$ as the principal's gross benefit from action $a$. The principal's expected utility (or surplus) is the expected gross benefit minus the expected payment: 
\begin{align*}
V_P(w(\cdot), F(\cdot)) = u(a^*) - \Ex_{x \sim F(a^*)}[w(x)],
\end{align*}

The timing of the interaction is as follows:
\begin{enumerate}
    \item The principal offers a contract $w: \mathcal{X} \to \mathbb{R}^+$.
    \item The agent chooses effort $a^* \in \mathcal{A}$ to maximize $V_A(a; w(\cdot), F(\cdot))$. 
    \item An outcome $x \in \mathcal{X}$ is realized according to the distribution $F(a)$.
    \item The agent receives payment $w(x)$; the principal receives surplus $u(a) - w(x)$. 
\end{enumerate}

The signal space can either be discrete or continuous, our result works either way. We typically think of the agent's action space as being continuous, and assume compactness when necessary. 

\paragraph{Linear and Affine Contracts}

A \emph{linear contract} is parameterized by $\phi \in (\mathbb{R}^+)^d$ and specifies payment
\[
\phi(x) = \langle \phi, x \rangle = \sum_{i=1}^d \phi_i x_i.
\]

An \emph{affine contract} is parameterized by $\psi = (\psi_0, \psi_1, \ldots, \psi_d) \in \mathbb{R}^{d+1}$ and specifies payment
\[
\psi(x) = \psi_0 + \sum_{i=1}^d \psi_i x_i.
\]



% \szcomment{Explain the binary outcome setting first to ease them into unbiasedness? }
% We frequently illustrate our results in the \emph{binary outcome setting}, where $\mathcal{X} = \{0,1\}^d$. Each component $x_i \in \{0,1\}$ represents success or failure on dimension $i$. In this setting, the agent's action space is $\mathcal{A} = [0,1]^d$, and the action $a_i$ represents the \emph{success probability} on dimension $i$:
% \[
% \Pr(x_i = 1 \mid a) = a_i.
% \]
% The condition $\Ex[x|a] = a$ is then definitional—it simply states that the agent chooses the marginal success probabilities. The joint distribution of outcomes across dimensions is left unspecified; this is precisely the source of distributional uncertainty.

% \begin{remark}
% Cross-task interactions enter the model through two channels: the cost function $c(a)$, which may exhibit complementarities or substitutabilities across dimensions, and the joint distribution of outcomes, which is part of the distributional uncertainty. The condition $\Ex[x_i|a] = a_i$ restricts only marginals, not the joint distribution.
% \end{remark}

% The condition $\Ex[x] = a$ is without loss of generality. Given any model with $\Ex[x|a] = f(a)$ for a monotone function $f$, one can relabel actions as $a' = f(a)$ to obtain $\Ex[x|a'] = a'$. This relabeling redefines the cost function as $\tilde{c}(a') = c(f^{-1}(a'))$ but does not restrict the economic environment. In the binary outcome setting discussed below, the condition is not even a normalization—it is definitional. 

% Given a contract $w(\cdot)$ and a compatible mapping ${F}(\cdot)$, let $a^*(w; {F}(\cdot)) \in \arg\max_{a \in \mathcal{A}} \Ex_{x \sim F(a)}[w(x)] - c(a)$ denote the agent's best response. 


% The framework above encompasses several economic settings:

% \begin{itemize}
%     \item \textbf{Multitask contracting} (Section~\ref{sec:multitask}): A single principal contracts with a single agent who exerts effort across $d$ tasks. Here $a_i$ represents effort on task $i$, and $x_i$ is the signal from task $i$.
    
%     \item \textbf{Common agency} (Section~\ref{sec:commonagency}): Multiple principals contract with a single agent. Each principal $j$ offers a contract $w_j$, and the agent responds to the aggregate incentives. 
    
%     \item \textbf{Team production} (Section~\ref{sec:teamproduction}): A single principal contracts with multiple agents who jointly contribute to a common output. Each agent $i$ chooses effort $a_i$ and receives contract $w_i$.
% \end{itemize}







==> sec/robustness.tex <==
% \section{Robustness of Linear Contracts}
% \label{sec:robustness}

% We consider a principal who faces \emph{distributional uncertainty}: she knows only the mean outcome $\Ex[x|a]$ for each action $a$, but not the full distribution of signals. The principal is ambiguity-averse and seeks to maximize her worst-case payoff over all distributions consistent with the known means. We introduce the notion of compatible distributions. 
% \begin{definition}[Compatible Distributions]
% A distribution mapping $F(a): \cA\mapsto \Delta(\cX)$ is \emph{compatible} if for each $a \in \mathcal{A}$,
% \[
% \Ex_{x \sim F(a)}[x | a] = a.
% \]
% \end{definition}
% \begin{remark}[Generality of the Mean Structure]
% Our definition above assumes $\Ex[x \mid a] = a$, which may appear to require unbiasedness. This is not essential. Our results extend to any known mean structure $\Ex[x \mid a] = \mu(a)$ satisfying mild regularity conditions—for example, $\mu$ concave in $a$. The proofs require only straightforward modifications. What is crucial is that the principal knows the mean outcome as a function of effort, not necessarily that effort and expected outcome coincide. We only choose this specific form to simplify the exposition. 
% \end{remark}

% The principal's \emph{worst-case payoff} from contract $w$ is
% \begin{align}
% {V}_P(w(\cdot)) = \min_{{F} \text{ compatible}} V_P(w(\cdot); {F}(\cdot)). \label{eq:robustnessObj}
% \end{align}

% The principal's problem is to choose a contract $w$ to maximize this worst-case payoff:
% \[
% \max_{w: \mathcal{X} \to \mathbb{R}^+} {V}_P(w(\cdot)).
% \]


% % To give some intuition, consider the binary outcome setting with $d$ tasks, so that $\mathcal{X} = \set{0,1}^d$. Now, the agent's effort vector $a$ determines the marginal success probability for each task and the signal satisfies: $\Ex[x|a] = a$. Any distribution mapping $F(\cdot)$ abiding the marginal success probability is compatible, however there is uncertainty about the behavior of the joint distribution. 

% We can now establish main robustness result for linear contracts under distributional ambiguity in the multitasking setting. We show that among all contracts, there exists a linear contract that maximizes the principal's worst-case objective. Our proof introduces a geometric approach based on \emph{self-inducing actions} and a concavification argument. Interestingly, our notion of \emph{self-inducing} actions also have a fixed-point interpretation. 

% \begin{theorem}[Robustness of Linear Contracts]
% \label{thm:robustness}
% Suppose $\mathcal{A}$ is compact. For any contract $w: \mathcal{X} \to \mathbb{R}_+$, there exists a linear contract $\phi \in (\mathbb{R}_+)^d$ such that
% \[
% V_P(\phi) \geq V_P(w).
% \]
% Further, there exists a linear contract $\phi^*$ maximizing $V_P(\phi)$. 
% \end{theorem}


% %%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Analysis Overview}
% \label{subsec:analysis-overview}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/robust-figure.pdf}
%     \caption{$w$ represents the contract, a function mapping outcome $x$ to a payment. We find $\psi^\sharp$, an upper supporting hyperplane to $w$. At the point $a^\sharp$, the marginal cost of the agent coincide with the slope of $\psi^\sharp$, hence $a^\sharp$ is induced under the affine contract $\psi^\sharp$. }
%     \label{fig:placeholder}
% \end{figure}


% We now give an overview of the analysis of our main robustness result (Theorem~\ref{thm:robustness}). We begin with the following observation. 

% \begin{observation}
% \label{obs:affine-invariance}
% Let $F$ be a compatible distribution mapping, then under an affine contract $\psi(x) = \psi_0 + \sum_{i=1}^d \psi_i x_i$, the agent's expected utility for any action $a$ is
% \[
% V_A(a; \psi) = \sum_{i=1}^d \psi_i \cdot a_i + \psi_0 - c(a),
% \]
% which depends only on the action $a$ and not on the particular compatible distribution mapping ${F}$.
% \end{observation}

% This observation implies that the principal's payoff under an affine contract is invariant across all compatible distribution mappings. Therefore, we aim to show that for any contract $w(\cdot)$, we can construct an affine contract $\psi$ and a specific compatible distribution mapping ${F}$ such that $V_P(\psi; {F}) \geq V_P(w; {F})$. By Observation~\ref{obs:affine-invariance}, this implies $V_P(\psi) \geq V_P(w)$, establishing that affine contracts are worst-case optimal. 

% Our proof strategy now works as follows. We introduce the key notion of a \emph{self-inducing} action and show how our problem boils down to showing existence of a \emph{self-inducing} action. Then, the existence of such an action can be shown via a geometric argument; interestingly, such actions also have a fixed-point interpretation. Finally, we show that any affine contract can be improved to a linear contract with weakly lower payment. 

% \subsection{Concavification of a non-affine contract}
% Let $w(\cdot)$ be any contract. We define the \emph{concave envelope} of $w$ as
% \[
% \overline{w}(a) = \sup \left\{ \sum_i \lambda_i w(x_i) : \lambda_i \geq 0, \; \sum_i \lambda_i = 1, \; \sum_i \lambda_i x_i = a \right\}.
% \]
% The concave envelope $\overline{w}(a)$ represents the maximum expected payment the agent can receive when taking action $a$, over all compatible distribution mappings. This is because any compatible distribution for action $a$ must have mean $a$, and can be expressed as a convex combination of outcomes in $\mathcal{X}$.

% For each action $a$, consider the set of supergradients (i.e. the superdifferential) of $\overline{w}(\cdot)$ at $a$. Each supergradient corresponds to an upper-supporting hyperplane to the graph of $\overline{w}(\cdot)$. 
% Each hyperplane $H$ that supports $\overline{w}(\cdot)$ from above naturally defines an affine contract $\psi(H)$ satisfying
% \[
% \psi_H(x) \geq w(x) \quad \text{for all } x \in \mathcal{X}.
% \]
% Thus, $\psi_H(\cdot)$ upper bounds the original payment function $w(\cdot)$.

% \subsection{Key Notion: Self-inducing Actions}
% The key concept in our proof is a \emph{self-inducing action}.

% \begin{definition}[Self-Inducing Action]
% \label{def:self-inducing}
% An action $a \in \mathcal{A}$ is \emph{self-inducing} if there exists an affine contract $\psi$ such that:
% \begin{enumerate}
%     \item $\psi$ induces action $a$ (i.e., $a$ is the agent's best response under $\psi$), and
%     \item $\psi$ supports $\overline{w}(\cdot)$ at the point $a$ from above, so that $\psi_H(\cdot) \ge w(\cdot)$ and $\psi(a) = \overline{w}(a)$. 
% \end{enumerate}
% \end{definition}


% Let $\psi^\sharp$ be the affine contract that induce $a^\sharp$ and also acts as the hyperplane supporting $\overline{w}(\cdot)$ at $a^\sharp$ from above. Recall at the concave envelope
% \[
% \overline{w}(a^\sharp) = \max\set{\sum_k \lambda_k w(x_k): \lambda_k > 0, \sum_k \lambda_k  = 1, \sum_k \lambda_k x_k = a^\sharp }. 
% \]
% Take $a^\sharp = \sum_k \lambda_k x_k$ as the optimal representation realizing the value of $\overline{w}(a^\sharp)$ as above. We then have
% \[
% \psi^\sharp(a^\sharp) = \sum_k \lambda_k \psi(x_k) \ge \sum_k \lambda_k \overline{w}(x_k) = w(a) = \psi^\sharp(a^\sharp). 
% \]
% The conclusion is of course that $\psi^\sharp(x_k) = \overline{w}(x_k)$ on all the ``support" points $x_k$. 

% Suppose that we have found a \emph{self-inducing} action $a^\sharp$. We construct a compatible distribution mapping $F(\cdot)$ as follows. For the action $a^\sharp$, we put the support onto $x_k$ as chosen above. For any other action $a$ we can choose any distribution that is compatible. Now, by taking the action $a^\sharp$ the agent receives identical payments under $\psi^\sharp$ and $w$, and for any action the payment under $w$ cannot be greater than $\psi^\sharp$. Since $\psi^\sharp$ induced $a^\sharp$, the contract $w$ would also induce $a^\sharp$ under $F(\cdot)$. Therefore under this distribution, the affine contract $\psi^\sharp$ performs as well as $w$. Since behavior of affine contracts are invariant across all compatible distributions, this means that $\psi^\sharp$ would be no worse-off than $w$ for the worst distribution. 

% % The significance of self-inducing actions is that they allow us to construct an affine contract $\psi$ and a compatible distribution under which $w$ performs exactly as well as $\psi$. Specifically, let $a$ be self-inducing, let $H$ be the corresponding upper-supporting hyperplane (so $\psi(H)$ is a supergradient at $\overline{w}(a)$), and suppose $\psi(H)$ induces $a$. We construct a compatible distribution for action $a$ that is concentrated on $P(H)$. Since $\psi(H)(x) = w(x)$ for all $x \in P(H)$ (by definition of the contact set), the agent receives identical expected payments under both contracts when taking action $a$. Moreover, since $\psi(H)$ upper bounds $w(\cdot)$ everywhere, if $\psi(H)$ induces action $a$, then $w(\cdot)$ must also induce $a$ under this distribution---any deviation would yield weakly lower payment under $w$ than under $\psi(H)$.

% % This means the principal achieves the same utility under $w$ as under $\psi(H)$ for this particular distribution family. Hence, finding a self-inducing action suffices to establish that $w(\cdot)$ can be improved to an affine contract with no worse worst-case utility.

% \subsection{Existence of Self-Inducing Actions.}
% We provide two approaches towards showing the existence of a self-inducing action. 

% \emph{Convex Minimization Approach. } We first give a characterization of \emph{self-inducing} actions. 

% \begin{proposition}[Characterization of Self-Inducing Actions]
% \label{prop:self-inducing-characterization}
% An action $a \in \mathcal{A}$ is self-inducing if and only if 
% \[
% \partial^- c(a) \cap \partial^+ \overline{w}(a) \neq \varnothing,
% \]
% where $\partial^-$ and $\partial^+$ denotes the subdifferential and superdifferential respectively.
% \end{proposition}
% \begin{proof}
% An affine contract $\psi$ induces action $a$ if and only if 
% $\psi_{1:d} \in \partial c(a)$ (the agent's first-order optimality 
% condition). Meanwhile, $\psi$ corresponds to a supergradient of 
% $\overline{w}$ at $a$ if and only if $\psi_{1:d} \in \partial \overline{w}(a)$. 
% The result follows immediately.
% \end{proof}
% By \Cref{prop:self-inducing-characterization}, we seek an action with $\partial^- c(a) \cap \partial^+ \overline{w}(a) \neq \varnothing$. Hence, consider the following convex minimization problem
% \[
% \min_a c(a) - \overline{w}(a). 
% \]
% Letting the minimizer be $a^\sharp$, then we have $0\in \partial^- [c(a^\sharp) - \overline{w}(a^\sharp)]$. 

% \emph{Fixed-point Approach. }
% The existence of a self-inducing action also follows from a fixed-point argument; the approach is less direct than the convex minimization perspective, however it shows that self-inducing actions exhibits some interesting topological aspect. For any action $a \in \mathcal{A}$, let $\mathcal{H}_{\mathrm{super}}(a)$ denote the set of upper-supporting hyperplanes that are supergradients at $\overline{w}(a)$. For any hyperplane $H$ corresponding to a valid affine contract (i.e., $H$ is non-vertical), let $a(H)$ denote the action induced by the affine contract $\psi(H)$.

% We define a set-valued mapping $g: \mathcal{H} \rightrightarrows \mathcal{H}$ on the space of upper-supporting hyperplanes by
% \[
% g(H) = \mathcal{H}_{\mathrm{super}}(a(H)).
% \]
% In words, $g(H)$ maps a hyperplane $H$ to the set of supergradients at the point $\overline{w}(a(H))$---that is, the supergradients at the concave envelope evaluated at the action that $H$ induces.

% By Kakutani's fixed-point theorem~\citep{kakutani1941generalization}, there exists a hyperplane $H^\sharp$ such that $H^\sharp \in g(H^\sharp)$. The action $a^\sharp = a(H^\sharp)$ is then precisely a self-inducing action: the affine contract $\psi(H^\sharp)$ both induces $a^\sharp$ and is a supergradient at $\overline{w}(a^\sharp)$. 

% \paragraph{Step 4: From affine to linear.}
% Once we have identified the self-inducing action $a^\sharp$, we know that the affine contract $\psi^\sharp$ achieves worst-case utility at least as good as $w$. By examining the agent's first-order conditions, we can show that any affine contract can be improved to a linear contract with at least weakly lesser payment while inducing the same action. 

% \subsection{Proof}
% Following the analysis given previously, we break the proof of \Cref{thm:robustness} to three lemmas: (1) existence of a self-inducing action, (2) construction of a distribution under which the affine contract performs at least as well as the original contract, and (3) refinement from affine to linear contracts.

% \begin{lemma}[Existence of Self-Inducing Action]
% \label{lem:self-inducing-exists}
% For any contract $w: \mathcal{X} \to \mathbb{R}_+$, there exists a self-inducing action $a^\sharp \in \mathcal{A}$.
% \end{lemma}

% \begin{proof}
% Consider the optimization problem
% \[
% \min_{a \in \mathcal{A}} \left[ c(a) - \overline{w}(a) \right].
% \]


% First note that a minimizer indeed exists. The function $c(a)$ is strictly convex and $\overline{w}(a)$ is concave (as the concave envelope of $w$). Hence the objective $c(a) - \overline{w}(a)$ is strictly convex. Since the domain $\mathcal{A} = \mathrm{conv}(\mathcal{X})$ is compact, a minimizer exists. 

% % In the continuous outcome setting with bounded growth, we have $\overline{w}(a) \leq C_1 \|a\|_1 + C_0$ for some constants $C_0, C_1$. Since $c(a)$ grows superlinearly (being strictly convex with $c(0) = 0$), the objective is coercive: $c(a) - \overline{w}(a) \to +\infty$ as $\|a\| \to \infty$. Hence a minimizer exists.

% % Let $a^\sharp$ denote a minimizer.

% Denote $\partial^{-}$ the subdifferential (for convex functions), $\partial^{+}$ the superdifferential (for concave functions). Now, at the minimizer $a^\sharp$, we have $0 \in \partial^{-}\ [c(a) - \overline{w}(a)]$. Hence $\partial^{-} c(a) \cap \overline{w}(a) \neq \varnothing$. This precisely means that $a^\sharp$ is self-inducing. 
% \end{proof}


% \begin{lemma}[Distribution for Self-Inducing Actions]
% \label{lem:self-inducing-distribution}
% Let $a^\sharp$ be a self-inducing action with corresponding affine contract $\psi^\sharp$ (i.e., $\psi^\sharp$ induces $a^\sharp$ and $\psi^\sharp$ is a supergradient of $\overline{w}$ at $a^\sharp$). There exists a compatible distribution $F$ such that:
% \begin{enumerate}
%     \item[(i)] The contract $w$ induces action $a^\sharp$ under $F$.
%     \item[(ii)] $\mathbb{E}_{x \sim F(a^\sharp)}[w(x)] = \mathbb{E}_{x \sim F(a^\sharp)}[\psi^\sharp(x)]$.
% \end{enumerate}
% \end{lemma}

% \begin{proof}
% Let $\psi^\sharp$ support $\overline{w}(a^\sharp)$ from above. 

% Define the contact set
% \[
% P = \{x \in \mathcal{X} : \psi^\sharp(x) = w(x)\},
% \]
% which consists of outcomes where the affine contract $\psi^\sharp$ touches the original contract $w$. Since $\psi^\sharp$ is a supergradient of $\overline{w}$ at $a^\sharp$, we have $a^\sharp \in \mathrm{conv}(P)$.

% Write $a^\sharp = \sum_{x \in P} \lambda_x x$ for some $\lambda_x \geq 0$ with $\sum_{x \in P} \lambda_x = 1$. Define the distribution $F$ by setting $F(a^\sharp)$ to be supported on $P$ with $\Pr(x) = \lambda_x$. Then $\mathbb{E}_{F(a^\sharp)}[x] = a^\sharp$, so $F$ is compatible.

% For any action $a \in \mathcal{A}$, the agent's payoff under $w$ is at most $\overline{w}(a) - c(a)$ (since $\overline{w}(a)$ is the maximum expected payment over all compatible distributions for action $a$). Since $\phi \in \partial^{+} \overline{w}(a^\sharp)$:
% \[
% \overline{w}(a) \leq \overline{w}(a^\sharp) + \langle \phi, a - a^\sharp \rangle.
% \]
% Since $\phi \in \partial^{-} c(a^\sharp)$:
% \[
% c(a) \geq c(a^\sharp) + \langle \phi, a - a^\sharp \rangle.
% \]
% Combining:
% \[
% \overline{w}(a) - c(a) \leq \overline{w}(a^\sharp) - c(a^\sharp), 
% \]
% and the inequality is strict for any $a \neq a^\sharp$. 

% At action $a^\sharp$ under distribution $F(a^\sharp)$, the agent's payoff is exactly $\mathbb{E}_{F(a^\sharp)}[w(x)] - c(a^\sharp)$. Since $F(a^\sharp)$ is supported on $P$ where $w(x) = \psi(x)$:
% \[
% \mathbb{E}_{F(a^\sharp)}[w(x)] = \mathbb{E}_{F(a^\sharp)}[\psi(x)] =  \overline{w}(a^\sharp).
% \]
% Thus the agent's payoff at $a^\sharp$ equals $\overline{w}(a^\sharp) - c(a^\sharp)$, which is maximal. Hence $w$ induces $a^\sharp$ under $F$. 
% \end{proof}

% The below lemma shows that if the principal were to induce some action $a$, then among all affine contracts, the linear contract $\phi$ would induce $a$ at least cost. The proof is deferred to \Cref{proof:affine-to-linear}. 
% \begin{lemma}[Adapted from Lemma 9 in \cite{roth2016watch}]
% \label{lem:best-linear}
% Suppose the agent's action set $\mathcal{A}$ is downward-closed, meaning if $a \in \mathcal{A}$, then $\rho a \in \mathcal{A}$ for all $\rho \in (0,1)$. Among all non-negative affine contracts that induce a given action $a$, the linear contract $\phi = \nabla c(a)$ induces $a$ with the minimum expected payment to the agent.
% \end{lemma}


% We can now collect all lemmas and prove our main robustness result. 
% \begin{proof}[{Proof of Theorem~\ref{thm:robustness}}]
% Let $w: \mathcal{X} \to \mathbb{R}_+$ be any contract.

% By Lemma~\ref{lem:self-inducing-exists}, there exists a self-inducing action $a^\sharp$ with corresponding affine contract $\psi^\sharp$ such that $\psi$ induces $a^\sharp$ and $\psi^\sharp(x) \geq w(x)$ for all $x \in \mathcal{X}$. By Lemma~\ref{lem:self-inducing-distribution}, there exists a compatible distribution $F$ such that:
% \begin{itemize}
%     \item Both $w$ and $\psi^\sharp$ induce action $a^\sharp$ under $F$.
%     \item The principal's payoff satisfies $V_P(\psi^\sharp; F) \geq V_P(w; F)$.
% \end{itemize}


% Under any compatible distribution $F'$, the agent's expected payment from affine contract $\psi^\sharp$ when taking action $a$ is
% \[
% \mathbb{E}_{F'(a)}[\psi(x)] = \psi^\sharp_0 + \langle \psi^\sharp_{1:d}, \mathbb{E}_{F'(a)}[x] \rangle = \psi_0^\sharp + \langle \psi^\sharp_{1:d}, a \rangle.
% \]
% This depends only on $a$, not on the specific distribution $F'$. Therefore, the principal's worst-case payoff under $\psi^\sharp$ equals her payoff under any particular compatible distribution:
% \[
% V_P(\psi^\sharp) = V_P(\psi^\sharp; F).
% \]

% Then we have
% \[
% V_P(\psi^\sharp) = V_P(\psi^\sharp; F) \geq V_P(w; F) \geq \min_{F' \text{ compatible}} V_P(w; F') = V_P(w).
% \]

% By Lemma~\ref{lem:best-linear}, among all affine contracts inducing action $a^\sharp$, the linear contract $\phi = \nabla c(a^\sharp)$ achieves the minimum expected payment. Since both $\psi^\sharp$ and $\phi$ induce $a^\sharp$, and $\phi$ pays weakly less:
% \[
% V_P(\phi) = u(a^\sharp) - \langle \nabla c(a^\sharp), a^\sharp \rangle \geq u(a^\sharp) - (\langle \psi^\sharp_{1:d}, a^\sharp \rangle + \psi^\sharp_0) = V_P(\psi^\sharp).
% \]

% Combining all steps:
% \[
% V_P(\phi) \geq V_P(\psi^\sharp) \geq V_P(w).
% \]
% Since $w$ was arbitrary, linear contracts are optimal for the principal's worst-case objective. 
% \end{proof}


\section{Robustness of Linear Contracts}
We consider a principal who faces distributional uncertainty: she knows only the mean outcome $\E[x|a]$ for each action $a$, but not the full distribution of signals. The principal is ambiguity-averse and seeks to maximize her worst-case payoff over all distributions consistent with the known means. We introduce the notion of compatible distributions.
\begin{definition}[Compatible Distributions]
A distribution mapping $F(a) : \A \mapsto \Delta(\X)$ is \emph{compatible} if for each $a \in \A$,
\[
\E_{x \sim F(a)}[x \mid a] = a.
\]
\end{definition}
\begin{remark}[Generality of the Mean Structure]
Our definition above assumes $\E[x \mid a] = a$, which may appear to require unbiasedness. This is not essential. Our results extend to any known mean structure $\E[x \mid a] = \mu(a)$ satisfying mild regularity conditions---for example, $\mu$ concave in $a$. The proofs require only straightforward modifications. What is crucial is that the principal knows the mean outcome as a function of effort, not necessarily that effort and expected outcome coincide. We only choose this specific form to simplify the exposition.
\end{remark}
The principal's worst-case payoff from contract $w$ is
\begin{equation}\label{eq:worst-case}
V_P(w(\cdot)) = \min_{F \text{ compatible}} V_P(w(\cdot); F(\cdot)).
\end{equation}
The principal's problem is to choose a contract $w$ to maximize this worst-case payoff:
\[
\max_{w: \X \to \R_+} V_P(w(\cdot)).
\]
We can now state our main result.
\begin{theorem}[Robustness of Linear Contracts]\label{thm:robustness}
Suppose $\A$ is compact. For any contract $w : \X \to \R_+$, there exists a linear contract $\phi \in (\R_+)^d$ such that
\[
V_P(\phi) \geq V_P(w).
\]
Further, there exists a linear contract $\phi^*$ maximizing $V_P(\phi)$.
\end{theorem}
The remainder of this section develops the proof. We proceed in four steps:
\begin{enumerate}[label=(\arabic*)]
    \item Establish that affine contracts are invariant across compatible distributions.
    \item Introduce the concave envelope and the key notion of self-inducing actions.
    \item Show that self-inducing actions exist and yield affine contracts that dominate arbitrary contracts in worst-case payoff.
    \item Refine from affine to linear contracts.
\end{enumerate}
%----------------------------------------------------------
\subsection{Step 1: Distribution Invariance of Affine Contracts}
%----------------------------------------------------------
We begin with a crucial observation that motivates our approach.
\begin{observation}\label{obs:invariance}
Let $F$ be a compatible distribution mapping. Under an affine contract $\psi(x) = \psi_0 + \sum_{i=1}^{d} \psi_i x_i$, the agent's expected utility for any action $a$ is
\[
V_A(a; \psi) = \sum_{i=1}^{d} \psi_i \cdot a_i + \psi_0 - c(a),
\]
which depends only on the action $a$ and not on the particular compatible distribution mapping $F$.
\end{observation}
This observation is immediate from the definition of compatible distributions: since $\E_{x \sim F(a)}[x] = a$ for any compatible $F$, the expected payment $\E[\psi(x)] = \psi_0 + \inner{\psi_{1:d}}{a}$ depends only on the mean.
The implication is powerful: the principal's payoff under an affine contract is invariant across all compatible distribution mappings. Therefore, our strategy is to show that for any contract $w(\cdot)$, we can construct an affine contract $\psi$ and a specific compatible distribution $F$ such that $V_P(\psi; F) \geq V_P(w; F)$. By \Cref{obs:invariance}, this implies $V_P(\psi) \geq V_P(w)$, establishing that affine contracts are worst-case optimal.
%----------------------------------------------------------
\subsection{Step 2: The Concave Envelope}
%----------------------------------------------------------
Let $w(\cdot)$ be any contract. We define the \emph{concave envelope} of $w$ as
\[
\wbar(a) = \sup \left\{ \sum_i \lambda_i w(x_i) : \lambda_i \geq 0, \sum_i \lambda_i = 1, \sum_i \lambda_i x_i = a \right\}.
\]
The concave envelope $\wbar(a)$ represents the maximum expected payment the agent can receive when taking action $a$, over all compatible distribution mappings. This is because any compatible distribution for action $a$ must have mean $a$, and can be expressed as a convex combination of outcomes in $\X$.
For each action $a$, consider the set of supergradients (i.e., the superdifferential) of $\wbar(\cdot)$ at $a$. Each supergradient corresponds to an upper-supporting hyperplane to the graph of $\wbar(\cdot)$. Each hyperplane $H$ that supports $\wbar(\cdot)$ from above naturally defines an affine contract $\psi_H$ satisfying
\[
\psi_H(x) \geq w(x) \quad \text{for all } x \in \X.
\]
Thus, $\psi_H(\cdot)$ upper bounds the original payment function $w(\cdot)$.
%----------------------------------------------------------
\subsection{Step 3: Self-Inducing Actions}
%----------------------------------------------------------
The key concept in our proof is a \emph{self-inducing action}---an action where the geometry of the concave envelope and the agent's cost function align perfectly.
\begin{definition}[Self-Inducing Action]\label{def:self-inducing}
An action $a \in \A$ is \emph{self-inducing} if there exists an affine contract $\psi$ such that:
\begin{enumerate}[label=(\roman*)]
    \item $\psi$ induces action $a$ (i.e., $a$ is the agent's best response under $\psi$), and
    \item $\psi$ supports $\wbar(\cdot)$ at the point $a$ from above, so that $\psi(x) \geq w(x)$ for all $x$ and $\psi(a) = \wbar(a)$.
\end{enumerate}
\end{definition}
Figure 1 illustrates this concept geometrically: at a self-inducing action $a^\sharp$, the upper-supporting hyperplane $\psi^\sharp$ to the concave envelope $\wbar$ has slope equal to the marginal cost $\nabla c(a^\sharp)$. This alignment ensures that $\psi^\sharp$ both induces $a^\sharp$ (via the agent's first-order condition) and touches $\wbar$ from above at $a^\sharp$.
The following characterization makes the definition concrete.
\begin{proposition}[Characterization of Self-Inducing Actions]\label{prop:characterization}
An action $a \in \A$ is self-inducing if and only if
\[
\subdiff c(a) \cap \supdiff \wbar(a) \neq \varnothing,
\]
where $\subdiff$ and $\supdiff$ denote the subdifferential and superdifferential respectively.
\end{proposition}
\begin{proof}
An affine contract $\psi$ induces action $a$ if and only if $\psi_{1:d} \in \partial c(a)$ (the agent's first-order optimality condition). Meanwhile, $\psi$ corresponds to a supergradient of $\wbar$ at $a$ if and only if $\psi_{1:d} \in \partial \wbar(a)$. The result follows immediately.
\end{proof}
Our first main lemma establishes that self-inducing actions always exist.
\begin{lemma}[Existence of Self-Inducing Action]\label{lem:existence}
For any contract $w : \X \to \R_+$, there exists a self-inducing action $a^\sharp \in \A$.
\end{lemma}
We provide two complementary perspectives on why this is true.
\paragraph{Convex Minimization Approach.}
By \Cref{prop:characterization}, we seek an action with $\subdiff c(a) \cap \supdiff \wbar(a) \neq \varnothing$. Consider the convex minimization problem
\[
\min_{a \in \A} \left[ c(a) - \wbar(a) \right].
\]
Since $c$ is strictly convex and $\wbar$ is concave, the objective is strictly convex. Compactness of $\A$ guarantees a minimizer $a^\sharp$. At this minimizer, the first-order condition $0 \in \subdiff[c(a^\sharp) - \wbar(a^\sharp)]$ implies $\subdiff c(a^\sharp) \cap \supdiff \wbar(a^\sharp) \neq \varnothing$, so $a^\sharp$ is self-inducing.
\paragraph{Fixed-Point Approach.}
The existence of a self-inducing action also follows from a fixed-point argument, revealing an interesting topological structure. For any action $a \in \A$, let $\Hcal_{\text{super}}(a)$ denote the set of upper-supporting hyperplanes that are supergradients at $\wbar(a)$. For any hyperplane $H$ corresponding to a valid affine contract (i.e., $H$ is non-vertical), let $a(H)$ denote the action induced by the affine contract $\psi(H)$.
Define a set-valued mapping $g: \Hcal \rightrightarrows \Hcal$ on the space of upper-supporting hyperplanes by
\[
g(H) = \Hcal_{\text{super}}(a(H)).
\]
In words, $g(H)$ maps a hyperplane $H$ to the set of supergradients at $\wbar(a(H))$---that is, the supergradients at the concave envelope evaluated at the action that $H$ induces.
By Kakutani's fixed-point theorem \cite{kakutani1941}, there exists a hyperplane $H^\sharp$ such that $H^\sharp \in g(H^\sharp)$. The action $a^\sharp = a(H^\sharp)$ is then precisely a self-inducing action: the affine contract $\psi(H^\sharp)$ both induces $a^\sharp$ and is a supergradient at $\wbar(a^\sharp)$.
%----------------------------------------------------------
\subsection{Step 4: Constructing the Dominating Distribution}
%----------------------------------------------------------
Given a self-inducing action, we can construct a specific compatible distribution under which the affine contract performs at least as well as the original contract.
\begin{lemma}[Distribution for Self-Inducing Actions]\label{lem:distribution}
Let $a^\sharp$ be a self-inducing action with corresponding affine contract $\psi^\sharp$ (i.e., $\psi^\sharp$ induces $a^\sharp$ and $\psi^\sharp$ is a supergradient of $\wbar$ at $a^\sharp$). There exists a compatible distribution $F$ such that:
\begin{enumerate}[label=(\roman*)]
    \item The contract $w$ induces action $a^\sharp$ under $F$.
    \item $\E_{x \sim F(a^\sharp)}[w(x)] = \E_{x \sim F(a^\sharp)}[\psi^\sharp(x)]$.
\end{enumerate}
\end{lemma}
The intuition is as follows. Let $\psi^\sharp$ be the affine contract that induces $a^\sharp$ and supports $\wbar(\cdot)$ at $a^\sharp$ from above. At the concave envelope,
\[
\wbar(a^\sharp) = \max \left\{ \sum_k \lambda_k w(x_k) : \lambda_k > 0, \sum_k \lambda_k = 1, \sum_k \lambda_k x_k = a^\sharp \right\}.
\]
Take $a^\sharp = \sum_k \lambda_k x_k$ as the optimal representation realizing $\wbar(a^\sharp)$. The key insight is that $\psi^\sharp(x_k) = w(x_k)$ on all the ``support'' points $x_k$---these are precisely the points where the supporting hyperplane touches the original contract.
We construct the compatible distribution $F(\cdot)$ by placing the distribution for action $a^\sharp$ onto these support points $x_k$. Under this distribution:
\begin{itemize}
    \item The agent receives identical payments under $\psi^\sharp$ and $w$ when taking action $a^\sharp$.
    \item For any other action, the payment under $w$ cannot exceed that under $\psi^\sharp$ (since $\psi^\sharp \geq w$ everywhere).
    \item Since $\psi^\sharp$ induces $a^\sharp$, the contract $w$ also induces $a^\sharp$ under $F(\cdot)$.
\end{itemize}
Therefore, under this distribution, the affine contract $\psi^\sharp$ performs as well as $w$. By \Cref{obs:invariance}, $\psi^\sharp$ achieves the same payoff under all compatible distributions, so $\psi^\sharp$ is no worse than $w$ even under the worst-case distribution.
%----------------------------------------------------------
\subsection{Step 5: From Affine to Linear Contracts}
%----------------------------------------------------------
The final step shows that any affine contract can be improved to a linear contract with weakly lower payment while inducing the same action.
\begin{lemma}[Linear Contracts Minimize Payment]\label{lem:linear}
Suppose the agent's action set $\A$ is downward-closed, meaning if $a \in \A$, then $\rho a \in \A$ for all $\rho \in (0,1)$. Among all non-negative affine contracts that induce a given action $a$, the linear contract $\phi = \nabla c(a)$ induces $a$ with the minimum expected payment to the agent.
\end{lemma}
The intuition is that the constant term $\psi_0$ in an affine contract is a ``wasteful'' payment---it does not contribute to incentives but increases the principal's cost. By setting $\psi_0 = 0$ and adjusting the linear coefficients appropriately, the principal can induce the same action at lower cost.
%----------------------------------------------------------
\subsection{Proofs}
%----------------------------------------------------------
We now provide the deferred proofs.
\begin{proof}[Proof of \Cref{lem:existence}]
Consider the optimization problem
\[
\min_{a \in \A} \left[ c(a) - \wbar(a) \right].
\]
First note that a minimizer exists. The function $c(a)$ is strictly convex and $\wbar(a)$ is concave (as the concave envelope of $w$). Hence the objective $c(a) - \wbar(a)$ is strictly convex. Since the domain $\A = \operatorname{conv}(\X)$ is compact, a minimizer exists.
Denote $\subdiff$ the subdifferential (for convex functions), $\supdiff$ the superdifferential (for concave functions). At the minimizer $a^\sharp$, we have $0 \in \subdiff[c(a) - \wbar(a)]$. Hence $\subdiff c(a) \cap \supdiff \wbar(a) \neq \varnothing$. This precisely means that $a^\sharp$ is self-inducing.
\end{proof}
\begin{proof}[Proof of \Cref{lem:distribution}]
Let $\psi^\sharp$ support $\wbar(a^\sharp)$ from above. Define the contact set
\[
P = \{x \in \X : \psi^\sharp(x) = w(x)\},
\]
which consists of outcomes where the affine contract $\psi^\sharp$ touches the original contract $w$. Since $\psi^\sharp$ is a supergradient of $\wbar$ at $a^\sharp$, we have $a^\sharp \in \operatorname{conv}(P)$.
Write $a^\sharp = \sum_{x \in P} \lambda_x x$ for some $\lambda_x \geq 0$ with $\sum_{x \in P} \lambda_x = 1$. Define the distribution $F$ by setting $F(a^\sharp)$ to be supported on $P$ with $\Pr(x) = \lambda_x$. Then $\E_{F(a^\sharp)}[x] = a^\sharp$, so $F$ is compatible.
For any action $a \in \A$, the agent's payoff under $w$ is at most $\wbar(a) - c(a)$ (since $\wbar(a)$ is the maximum expected payment over all compatible distributions for action $a$). Since $\phi \in \supdiff \wbar(a^\sharp)$:
\[
\wbar(a) \leq \wbar(a^\sharp) + \inner{\phi}{a - a^\sharp}.
\]
Since $\phi \in \subdiff c(a^\sharp)$:
\[
c(a) \geq c(a^\sharp) + \inner{\phi}{a - a^\sharp}.
\]
Combining:
\[
\wbar(a) - c(a) \leq \wbar(a^\sharp) - c(a^\sharp),
\]
and the inequality is strict for any $a \neq a^\sharp$.
At action $a^\sharp$ under distribution $F(a^\sharp)$, the agent's payoff is exactly $\E_{F(a^\sharp)}[w(x)] - c(a^\sharp)$. Since $F(a^\sharp)$ is supported on $P$ where $w(x) = \psi(x)$:
\[
\E_{F(a^\sharp)}[w(x)] = \E_{F(a^\sharp)}[\psi(x)] = \wbar(a^\sharp).
\]
Thus the agent's payoff at $a^\sharp$ equals $\wbar(a^\sharp) - c(a^\sharp)$, which is maximal. Hence $w$ induces $a^\sharp$ under $F$.
\end{proof}
\begin{proof}[Proof of \Cref{lem:linear}]
Adapted from Lemma 9 in \cite{roth2016watch}. The proof is deferred to the appendix.
\end{proof}
\begin{proof}[Proof of \Cref{thm:robustness}]
Let $w : \X \to \R_+$ be any contract.
By \Cref{lem:existence}, there exists a self-inducing action $a^\sharp$ with corresponding affine contract $\psi^\sharp$ such that $\psi$ induces $a^\sharp$ and $\psi^\sharp(x) \geq w(x)$ for all $x \in \X$. By \Cref{lem:distribution}, there exists a compatible distribution $F$ such that:
\begin{itemize}
    \item Both $w$ and $\psi^\sharp$ induce action $a^\sharp$ under $F$.
    \item The principal's payoff satisfies $V_P(\psi^\sharp; F) \geq V_P(w; F)$.
\end{itemize}
Under any compatible distribution $F'$, the agent's expected payment from affine contract $\psi^\sharp$ when taking action $a$ is
\[
\E_{F'(a)}[\psi(x)] = \psi_0^\sharp + \inner{\psi_{1:d}^\sharp}{\E_{F'(a)}[x]} = \psi_0^\sharp + \inner{\psi_{1:d}^\sharp}{a}.
\]
This depends only on $a$, not on the specific distribution $F'$. Therefore, the principal's worst-case payoff under $\psi^\sharp$ equals her payoff under any particular compatible distribution:
\[
V_P(\psi^\sharp) = V_P(\psi^\sharp; F).
\]
Then we have
\[
V_P(\psi^\sharp) = V_P(\psi^\sharp; F) \geq V_P(w; F) \geq \min_{F' \text{ compatible}} V_P(w; F') = V_P(w).
\]
By \Cref{lem:linear}, among all affine contracts inducing action $a^\sharp$, the linear contract $\phi = \nabla c(a^\sharp)$ achieves the minimum expected payment. Since both $\psi^\sharp$ and $\phi$ induce $a^\sharp$, and $\phi$ pays weakly less:
\[
V_P(\phi) = u(a^\sharp) - \inner{\nabla c(a^\sharp)}{a^\sharp} \geq u(a^\sharp) - \left( \inner{\psi_{1:d}^\sharp}{a^\sharp} + \psi_0^\sharp \right) = V_P(\psi^\sharp).
\]
Combining all steps:
\[
V_P(\phi) \geq V_P(\psi^\sharp) \geq V_P(w).
\]
Since $w$ was arbitrary, linear contracts are optimal for the principal's worst-case objective.
\end{proof}



% \begin{remark}[Topological Perspective]
% \label{rem:kakutani}
% An alternative proof of Lemma~\ref{lem:self-inducing-exists} uses Kakutani's fixed-point theorem. Define the set-valued mapping $g: \mathcal{H} \rightrightarrows \mathcal{H}$ on upper-supporting hyperplanes by $g(H) = \mathcal{H}_{\mathrm{super}}(a(H))$, where $a(H)$ is the action induced by the affine contract corresponding to $H$. A fixed point $H^* \in g(H^*)$ yields a self-inducing action $a^* = a(H^*)$. In the binary example of Section~\ref{subsec:example}, this fixed-point argument reduces to the intermediate value theorem. The minimization approach presented above provides a more direct argument while also yielding the characterization in Proposition~\ref{prop:self-inducing-characterization}.
% \end{remark}

% \begin{lemma}
% \label{lem:best-linear}
% Suppose the agent's action set $\mathcal{A}$ is downward-closed (i.e., if $a \in \mathcal{A}$ then $\rho a \in \mathcal{A}$ for all $\rho \in (0,1)$). Among all non-negative affine contracts that induce a given action $a$, the linear contract $\phi = \nabla c(a)$ induces $a$ with the minimum expected payment to the agent.
% \end{lemma}

% Applying Lemma~\ref{lem:best-linear}, if $\psi(H^*)$ induces action $a^*$, then the linear contract $\phi = \nabla c(a^*)$ also induces $a^*$ at weakly lower payment. This completes the proof: starting from an arbitrary contract $w$, we have identified a linear contract achieving worst-case utility at least as high as $w$. Since $w$ was arbitrary, linear contracts are optimal in the worst-case sense.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{An Example with Binary Outcomes}
% \label{subsec:binary-example}

% We illustrate the proof through a concrete example. Consider a setting with $d = 2$ tasks and the following non-linear contract $w$ defined on $\mathcal{X} = \{0,1\}^2$:
% \[
% w(0,0) = 0, \quad w(1,0) = 2, \quad w(0,1) = 2, \quad w(1,1) = 3.
% \]
% We trace how our proof identifies an improvement from $w(\cdot)$ to a linear contract.

% \paragraph{Upper concave envelope.}
% If $w(\cdot)$ were affine, then the graph of the mapping $\{(x, w(x)) : x \in \mathcal{X}\} \subset \mathbb{R}^3$ would lie on a single hyperplane. We see that $w(\cdot)$ is not affine, and the upper concave envelope comprises two facets. 

% The first upper facet $H_1$ touches $\mathcal{X}$ at the points $\mathcal{X}_1 = \{(0,0), (1,0), (0,1)\}$ and corresponds to an affine contract $\psi(H_1)$ with values:
% \[
% \psi(H_1)(0,0) = 0, \quad \psi(H_1)(1,0) = 2, \quad \psi(H_1)(0,1) = 2, \quad \psi(H_1)(1,1) = 4.
% \]

% The second upper facet $H_2$ touches $\mathcal{X}$ at $\mathcal{X}_2 = \{(1,0), (0,1), (1,1)\}$ and corresponds to an affine contract $\psi(H_2)$ with values:
% \[
% \psi(H_2)(0,0) = 1, \quad \psi(H_2)(1,0) = 2, \quad \psi(H_2)(0,1) = 2, \quad \psi(H_2)(1,1) = 3.
% \]

% \paragraph{Self-inducing actions.}
% Consider an action $a \in \conv(\mathcal{X}_1)$. If the affine contract $\psi(H_1)$ induces $a$, then $a$ is \emph{self-inducing}. Similarly, for an action $a \in \conv(\mathcal{X}_2)$, if $\psi(H_2)$ induces $a$, then $a$ is self-inducing.

% There is also a third possibility. Any convex combination $H_\lambda = \lambda H_1 + (1-\lambda) H_2$ for $\lambda \in [0,1]$ defines a valid upper supporting hyperplane. This hyperplane is supported on the segment with endpoints $(1,0)$ and $(0,1)$---the intersection $\conv(\mathcal{X}_1) \cap \conv(\mathcal{X}_2)$. For an action $a$ belonging to this segment, if some $H_\lambda$ induces $a$, then $a$ is also self-inducing.

% \paragraph{Existence of self-inducing actions.}
% Suppose for the sake of contradiction that $\psi(H_1)$ induces an action in $\conv(\mathcal{X}_2) \setminus \conv(\mathcal{X}_1)$ and that $\psi(H_2)$ induces an action in $\conv(\mathcal{X}_1) \setminus \conv(\mathcal{X}_2)$. (Otherwise, we would already have found a self-inducing action.)

% Observe that the map from hyperplanes to induced actions is continuous: small perturbations in the contract lead to small changes in the agent's best response. As we continuously interpolate from $H_1$ to $H_2$ via $H_\lambda = \lambda H_1 + (1-\lambda) H_2$, the induced action moves continuously from $\conv(\mathcal{X}_2)$ to $\conv(\mathcal{X}_1)$. At some intermediate value $\lambda^* \in (0,1)$, the induced action must lie exactly on the segment between $(1,0)$ and $(0,1)$. Hence, a self-inducing action exists. In this example, Kakutani's fixed-point theorem manifests as the intermediate value theorem.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Extension to Continuous Outcome Spaces}
% \label{subsec:continuous-extension}

% We now extend Theorem~\ref{thm:robustness} to continuous outcome spaces. In fact, we give an exact characterization of self-inducing actions. 

% In this setting, we require a bounded-growth condition on contracts.

% \begin{definition}[Bounded Growth]
% \label{def:bounded-growth}
% A function $f: (\mathbb{R}_+)^d \to \mathbb{R}_+$ has \emph{bounded growth} if there exist constants $C_0, C_1 \geq 0$ such that $f(x) \leq C_1 \|x\|_1 + C_0$ for all $x$.
% \end{definition}

% \begin{theorem}[Robustness with Continuous Outcomes]
% \label{thm:robustness-continuous}
% Let $\mathcal{A} = \mathcal{X} = (\mathbb{R}_+)^d$. For any contract $w: \mathcal{X} \to \mathbb{R}_+$ with bounded growth, there exists a linear contract $\phi \in (\mathbb{R}_+)^d$ such that
% \[
% V_P(\phi) \geq V_P(w).
% \]
% \end{theorem}

% The bounded-growth condition is necessary because if $w(\cdot)$ grows superlinearly (e.g., $w(x) = \|x\|_2^2$), then the upper concave envelope is not well-defined. However, if the principal's gross utility $u(a)$ has bounded growth---a natural assumption that prevents the optimal contract from inducing unbounded effort---then any contract without bounded growth cannot be optimal. We may therefore restrict attention to contracts with bounded growth without loss of generality. See Appendix~\ref{app:bounded-growth} for a more detailed argument. 

% The proof follows the same strategy as Theorem~\ref{thm:robustness}: we seek a self-inducing action. The key technical difference is that in the continuous setting, the supergradient of the concave envelope may not correspond to a valid (non-vertical) hyperplane at boundary points. For instance, if $w(x) = \sqrt{x}$, the supergradient at $x = 0$ is a vertical line, which does not define a valid affine contract.

% Let us examine \emph{self-inducing actions} once more. In fact, a self-inducing action corresponds exactly to an action which has:
% \[
% \partial c(a) \cap \partial \overline{w}(a) \neq \varnothing. 
% \]
% That is, the subgradient for the agent's cost function $c(\cdot)$ and the supergradient for the concave envelop $\overline{w}(\cdot)$ share a similar element. 

% \begin{proposition}
% If for some action $a$, [subgradient intersect supergradient] non empty, then $a$ is self-inducing. Further, we can find some point $a$ such that [subgradient intersect supergradient] non empty. 
% \end{proposition}
% \begin{proof}
% First show that a minimizer exists. If $a$ is in interior we are done. Otherwise suppose $a$ is on boundry with some coordinates equal to 0. 

% Then for non-zero coordinate we have coord equal in sub / supergradient. Otherwise we have the subgradient coord > supergradient coord. The economic interpration is of course that the marginal cost of inducing the action to invest a infitesmial amount effort outweights the marginal benefit, so that the optimal stays on the boundry. However, even in such case, we can increase the supergradient coord to be the same as the subgradient coord, and this new vector would still be a valid supergradient coord. 
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse

\section{Robustness of Linear Contracts in Multitasking (OLD)}

\szcomment{Claude's respones: "We establish that linear contracts are robust in multitasking environments—a setting of significant practical relevance. Our proof introduces a geometric approach based on self-owned hyperplanes and fixed-point arguments, which yields not only the multitask result but also extensions to common agency and team production. As a byproduct, this provides a simpler proof of the 1-D result of [Prior Work]." } 

In this section, we present our main robustness result for linear contracts under distributional ambiguity. We present our results in the multitasking setting. The crux of the proof is a geometric approach based on fixed-point arguments. 

% In this section, we assume that tasks generate binary signals, with the signal space denoted as $\mathcal{X} = \set{0,1}^d$. The agent's action space is given by $\mathcal{A} = [0,1]^d$. When the agent takes an action $a \in \mathcal{A}$, the expected signal for task $i$ is $a_i$, and the agent incurs a cost $c(a)$. 


Our main result establishes that among all contracts, there exists a linear contract that maximizes the worst-case objective.

%Recall that under the linear contract $\phi$, the agent's payment under signal $x$ is
% \[
% \phi(x) = \sum_{i=1}^d \phi_i x_i. 
% \]

\begin{theorem}[Robustness of Linear Contracts]
\label{thm:robustness}
Assume the signal space is finite. For any (possibly non-linear) contract $w(\cdot)$. There exists a linear contract $\phi$ such that
\[
V_P(\phi) \ge V_P(w). 
\]
% There exists a linear contract $\phi \in (\mathbb{R}^+)^d$ that maximizes the principal's worst-case objective~\eqref{eq:robustnessObj}. That is, there is a linear contract $\phi$ such that:
% \[
% V_P(\phi) = \max_{w: \mathcal{X} \to \mathbb{R}^+} V_P(w).
% \]
\end{theorem}



% Let's first examine how the proof works in 1-d. Let $w()$ be any contract, then its graph forms a curve in the 2-d plane. Now, the worst case payment for any action $a$ is the concave envelope
% \[
% xxx. 
% \]
% Consider any action $a$, and its set of supergradients of the concave envelope. We call an action \emph{invent a name, maybe self-inducing} if there exists a linear contract that induces $a$ and that the linear contract is in the supergradient set. If we can find a self-inducing $a$, then we are done: we construct a compatible distribution where the support of the signal when the agent takes action $a$ is supported on the supports of the upper supporting hyperplane (the supergradient) that touch the graph. 

\input{sec/analysis_overview}
% We now claim that there must exist at least one hyperplane among these—one that we call \emph{self-owned}—for which the induced action lies within its own set of support points (after projecting back to \(\mathcal{X}\)). In other words, if \(H\) is the hyperplane corresponding to an affine contract \(\phi(H)\), define
% \[
% P(H)=\{x\in \mathcal{X} \mid (x,w(x))\in H\}.
% \]
% Then \(H\) is \emph{self-owned} if the action \(a\) induced by \(\phi(H)\) satisfies
% \[
% a \in \operatorname{conv}(P(H)).
% \]



% The model we will be working with will be different from the previous sections which provided the uniformity result and ... Actions are distribution-ambiguous, meaning that $a\in\mathcal{A}$, the expected outcome 





%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%



% \subsection{Ambiguous in distribution for $d = 2$}

% Here we show robustness results in an ambiguous principal-agent setting. 



% We consider a setting where there are 2 tasks, and that either task can succeed or fail, so that there is a total of 4 outcomes. 



% We show that under an ambiguous principal-agent setting, the optimal contract must be of the form

% \[

% w(y) = \phi_0 + \phi_1 \ind{y_1 = 1} + \phi_2 \ind{y_2 = 1}. 

% \]



% \begin{theorem}

% Given an ambiguous principal agent setting with a set of actions $A$. Given any contract $w(\cdot)$, there exists a contract $\phi$ in the family of affine contracts, such that there exists a family of compatible distribution (recall distribution is for each action), such that the payoff of $\phi$ to the principal is no less than that of $w(\cdot)$. 

% \end{theorem}



% \begin{proof}

% There are two cases. First case is that $s(1,1) > s(0,0) + s(0,1) - s(0,0)$. 



% Second case is that $s(1,1) < s(1,0) + s(0,1) - s(0,0)$. 



% In the first case, we lower either the payoff for $s(1,1)$ or $s(0,0)$. And show that at least in one of the two affine contracts, the optimal action $a^*$'s payment in the 2 schemes will remain the same. This is because, at least in one of the two schemes, the action $a^*$ will be in the convex hull whose payoff did not change. 



% In the 2nd case, we lower either the payoff for $s(1,0)$ or $s(0,1)$. And show that at least in one of the two newly formed affine contracts, the optimal action $a^*$'s payment in the 2 schemes will remain the same. 

% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{An example with Binary Outcomes}
Let us illustrate the the proof through a concrete example. Consider a setting with $d=2$ tasks and the following non-linear contract $w$ defined on $\mathcal{X} = \{0,1\}^2$:
\[
w(0,0)=0,\quad w(1,0)=2,\quad w(0,1)=2,\quad w(1,1)=3.
\]
We trace how our proof identifies an improvement from $w(\cdot)$ to a linear contract. 

\paragraph{Upper Concave envelope. }
In general if $w(\cdot)$ were affine, then the polytope $(x, w(x))$ would lie on a hyperplane. For our example $w(\cdot)$ is not affine, and the concave envelope comprise of two factes. 

The first upper facet $H_1$ touches $\mathcal{X}$ at the points $\mathcal{X}_1 = \{(0,0),\, (1,0),\, (0,1)\}$, corresponds to an affine contract $\phi(H_1)$ with values
\[
\phi(H_1)(0,0)=0,\quad \phi(H_1)(1,0)=2,\quad \phi(H_1)(0,1)=2. 
\]

The second upper facet $H_2$ touches $\mathcal{X}$ at $\{(1,0),\, (0,1),\, (1,1)\}$, corresponding to an affine contract $\phi(H_2)$ with values: 
\[
\phi(H_2)(1,0)=2,\quad \phi(H_2)(0,1)=2,\quad \phi(H_2)(1,1)=3. 
\]

\paragraph{Self-inducing actions. }
Consider an action $a \in \conv{\cX_1}$. If the affine contract $\psi(H_1)$ induced $a_1$, then $a$ is self-inducing. Similarly for an action $a\in \conv{\cX_2}$, if the affine contract $\psi(H_2)$ induced $a$, then $a$ is self-inducing. There is also a third possibility. We know that any convex combination $H_\lambda = \lambda H_1 + (1-\lambda) H_2$ for $\lambda \in [0,1]$ also defines a valid upper supporting hyperplane supported on the segment with endpoints $()$ and $()$. For an action $a$ that belongs to this segment, if there is some $H_{\lambda}$ that induce this action, then $a$ would also be self-inducing. 

% Consider our two hyperplanes $H_1$ and $H_2$. If the action $a(H_1)$ falls in $\conv(\mathcal{X}_1)$, then $a(H_1)$ is self-inducing. If the action $a(H_2)$ falls in $\conv(\cX_2)$, then $a(H_2)$ is \emph{self-inducing}. 

% Any convex combination $H_\lambda = \lambda H_1 + (1-\lambda) H_2$ for $\lambda \in [0,1]$ also defines a valid upper supporting hyperplane. Such a combination is self-owned if its induced action lies on the intersection between $\conv(\mathcal{X}_1)$ and $\conv(\mathcal{X}_1)$, i.e., the interval with endpoint $(1,0)$ and $(0,1)$. 

\paragraph{Existense of self-inducing actions. }
Suppose for sake of contradiction that $\psi(H_1)$ induced an action in $\conv(\cX_2)$ and that $\psi(H_2)$ induced an action in $\conv(\cX_1)$; otherwise we would already have found the self-inducing action. 

% Returning to our running example once more, suppose, for contradiction, that neither $H_1$ nor $H_2$ is self-owned. Then $\phi_1$ induces an action in $\conv(X_2)$ (not in $\conv(X_1)$), while $\phi_2$ induces an action in $\conv(X_1)$ (not in $\conv(X_2)$). 

Note that the map from hyperplanes to induced actions is continuous—small perturbations in the contract lead to small changes in the agent's best response. As we continuously interpolate from $H_1$ to $H_2$ via $H_\lambda = \lambda H_1 + (1-\lambda) H_2$, the induced action must continuously move from $\conv(X_2)$ to $\conv(X_1)$. At some intermediate value $\lambda^* \in (0,1)$, the induced action must lie exactly on the segment with endpoints $()$ and $()$. Hence we have found the self-inducing action. In this example, Kakutani's theorem effectively manifests as the intermediate value theorem. 


\subsection{Extend to Continuous Outcome Space}
Here we extend the argument to continuous setting where $\mathcal{A} = \mathcal{X} = (\bR^+)^d$. We need to impose a bounded growth condition for our arguments to work. In particular, if $w(\cdot)$ grows faster than a linear function, for example $w(x) = \norm{x}_2^2$, then the upper concave envelope of $w(x)$ is not well defined. However, if the principal's gross utility $u(a)$ has bounded-growth (which is a natural condition, as it prevents the optimal contract from inducing an action that goes to $+\infty$), then any contract that does not have bounded growth cannot be optimal, so w.l.o.g. we can restrict attention to contracts with bounded growth. For discussion see Appendix ???. 

\begin{theorem}
Let $\mathcal{A} = (\mathbb{R}^+)^d$ and that $\mathcal{X} = (\mathbb{R}^+)^d$. Let $w(\cdot)$ be any contract mapping with bounded growth. There exists a linear contract $\phi$ and a compatible distribution mapping $\mathcal{F}$ such that 
\[
V_P(\phi) \ge V_P(w(\cdot), F(\cdot))
\]
\end{theorem}

The main idea is exactly same: finding self-inducing action. However, one issue in the continuous setting is that the supergradient may not correspond to valid hyperplanes at boundry points. For example $w(x) = \sqrt{x}$. The supergradient at the boundry $x = 0$ is the vertical line. We resolve this by showing existence by modifying the application of Kakutani's fixed-point theorem to an adaption of the intermediate value theorem. 

Each $a$ maps to a set of linear contracts that induce it. 

Each $a$ also maps to a set of supergradients. 

Need to show exists some $a$ such that $\phi(a) \in \mathcal{D}(a)$. There exists a continuous selection of supergradient. 



%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{Proof Idea}
% Let's first focus on affine contracts. We show that there exists an affine contract that maximizes the principal’s worst-case objective. A key property of affine contracts is that under any family of compatible distributions over outcomes, the agent’s best response remains unchanged---so the principal’s payoff is independent of the particular distribution in that family. Then in the last step, we improve the affine contract to a linear contract. 

We start with the following observation. 

\begin{observation}
The agent's payoff from an affine contract does not depend on the particular choice of distribution family \(\mathcal{F}\). 
% it follows that the worst-case objective achieved by some affine contract is at least as good as that achieved by \(w(\cdot)\). 
\end{observation}

Given any (possibly non-affine) contract \(w(\cdot)\), we will construct an affine contract \(\phi\) and identify a corresponding family of compatible distributions \(\mathcal{F}\) such that the principal’s payoff under \(\phi\) is at least as high as under \(w\) for the compatible distribution family \(\mathcal{F}\). Then by the previous observation, ...


We also consider a specific example when walking through the key ideas in the proof. For the concrete example, we consider a setting with \(d=2\) and the following non-affine (non-linear) contract \(w\) defined on \(\mathcal{X} = \{0,1\}^2\):
\[
w(0,0)=0,\quad w(1,0)=2,\quad w(0,1)=2,\quad w(1,1)=3.
\]
We tract how the proof finds a linear contract on this example. 

\paragraph{\bf A Family of Affine Contract via Upper Supporting Hyperplanes.} 
Consider the \emph{lifted set}
\[
S = \{ (x, w(x)) : x \in \mathcal{X} \}.
\]
For any hyperplane \(H\) that supports \(S\) from above (an \emph{upper supporting hyperplane}), we can associate an affine contract \(\phi(H)\) that satisfies $\phi(H) > w(x)$. In this way, \(\phi(H)\) serves as an upper bound to the payment function \(w\). To obtain the affine contract, we upper-bound \(w(\cdot)\) by finding an affine function \(\phi\) that satisfies
\[
\phi(x) \ge w(x) \quad \text{for all } x.
\]

\medskip
\textit{Tracing the Example. }
In our example, we \emph{lift} the space \(\mathcal{X}\) into \(\mathbb{R}^3\) by appending the contract payment value as a third coordinate. We have the lifted set as
\[
S = \{(0,0,0),\ (1,0,2),\ (0,1,2),\ (1,1,3)\}.
\]
If \(w\) were affine, then \(S\) would lie on a single hyperplane in \(\mathbb{R}^3\). Since \(w\) is not affine, \(S\) forms a polytope with several facets. In particular, there are two \emph{upper facets} of \(S\) that yield upper supporting hyperplanes, each corresponding to an affine contract that upper bounds \(w\).

One such upper facet defines an affine contract \(\phi_1\) with
\[
\phi_1(0,0)=0,\quad \phi_1(1,0)=2,\quad \phi_1(0,1)=2,\quad \phi_1(1,1)=4.
\]
This hyperplane touches \(S\) at the points
\[
X_1 = \{(0,0),\ (1,0),\ (0,1)\}.
\]
Similarly, another upper facet defines an affine contract \(\phi_2\) given by
\[
\phi_2(0,0)=1,\quad \phi_2(1,0)=2,\quad \phi_2(0,1)=2,\quad \phi_2(1,1)=3,
\]
supported on the points
\[
X_2 = \{(1,0),\ (0,1),\ (1,1)\}.
\]
Note that $\conv(X_1)$ and $\conv(X_2)$ are disjoint sets and that: $\mathcal{X} = \conv(X_1)\cup \conv(X_2)$. 

\medskip

\paragraph{\bf ``Self-Owned" Hyperplanes.} 
We now introduce the notion of a \emph{self-owned hyperplane}, which is the key concept in our proof. A hyperplane \(H\) is called \emph{self-owned} if the induced action \(a(H) = a(\phi(H))\) under the affine contract \(\phi(H)\) lies in the convex hull of its own contact set (after projected back to $\mathcal{X}$), that is,
\[
a(H) \in \operatorname{conv}(P(H)).
\]
Here we define
\[
P(H) = \{ x \in \mathcal{X} : (x, w(x)) \in H \}. 
\]
When \(H\) is self-owned, one may choose a compatible distribution where the support of taking action $a(H)$ is only supported on \(P(H)\). Then, since $H$ touches the $S$, we know that the agent’s payment is identical under both \(w\) and \(\phi(H)\). This means that if the affine contract $\phi(H)$ induced action $a$, then under this compatible distribution the non-affine contract $w(\cdot)$ also induces action $a$, and that $\phi(H)$ induces $a$ at a no larger payment. 

\textit{Tracing the example. }
In our example, recall that $H_1$ and $H_2$ are two supporting hyperplanes. Their convex combination are also valid supporting hyperplanes. Now, if the action induced by the hyperplane $H_1$ lies in $xx$, or if the action induced by the hyperplane $H_2$ lies in $xx$, then they would be self-owned. Also, for a convex combination, if the induced action lies in $xx$, then it is also self-owned. 

% For the affine contract \(\phi(H)\) to be effective, we need that for the action \(a\) chosen by the agent, the payment under \(\phi(H)\) coincides with that under \(w\), i.e.,
% \[
% \phi(H)(a) = w(a).
% \]
% This equality can be ensured if the distribution of outcomes when the agent takes action \(a\) lies entirely on the set of points where \(H\) touches \(S\). Define
% \[
% P(H) = \{ x \in \mathcal{X} : (x, w(x)) \in H \},
% \]
% as the projection of these contact points onto \(\mathcal{X}\).


\medskip

\paragraph{\bf Existence of a Self-Owned Hyperplane. } A classical result in convex geometry (e.g. \cite{lee2017subdivisions}) implies that the union of the convex hulls of \(P(H)\) over all upper supporting hyperplanes \(H\) covers the entire outcome space \(\mathcal{X}\). In particular, for every action \(a \in \mathcal{X}\) there exists some hyperplane \(H\) such that \(a \in \operatorname{conv}(P(H))\). Then, we can construct a set-valued mapping:
\[
g: \mathcal{H} \to 2^\mathcal{H},
\]
defined as
\[
g(H) = \set{H': a(H) \in \conv(P(H'))}. 
\]
By applying Kakutani's fixed point theorem (\cite{kakutani1941generalization}), there exists a hyperplane \(H^*\) such that
\[
H^* \in g(H^*).
\]
Then we have precisely found a self-owned hyperplane. 

\medskip \textit{Tracing the Example. }
Suppose, for the sake of contradiction, that no self-owned hyperplane exists. Then the affine contract \(\phi_1\) would induce an action falling in \(X_2\) while \(\phi_2\) would induce an action in \(X_1\). However, the mapping from the hyperplane to the induced action is continuous (small changes in the hyperplane lead to small changes in the induced action). Therefore, as one continuously interpolates between \(\phi_1\) and \(\phi_2\), the induced action must eventually lie exactly in the convex combination (or “interval”) determined by \((1,0)\) and \((0,1)\). Note that here Kakutani's fixed point theorem reduces to an intermediate value theorem. Hence, this guarantees the existence of a self-owned hyperplane. 

%This fixed point \(H^*\) is self-owned, meaning that the action incentivized by \(\phi(H^*)\) is supported on \(P(H^*)\). Consequently, by choosing a compatible distribution supported on \(P(H^*)\), the agent receives the same payment under both \(w\) and \(\phi(H^*)\).

\medskip

\paragraph{\bf Refining to a Linear Contract.} Finally, we show that if the affine contract \(\phi\) induces an action \(a^*\), then there exists a linear contract (i.e., one with zero offset) that also induces \(a^*\) while providing no greater payment to the agent. This completes the proof by establishing that within the class of contracts, a linear contract exists that maximizes the principal’s worst-case objective. 

\medskip

By these steps, we conclude that for any arbitrary contract \(w\), there is a linear contract that performs at least as well in the principal’s worst-case evaluation. This completes the proof sketch. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Remove my own proof idea
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Proof Idea}
% In this section, we briefly outline the idea behind the theorem. 

% We first show that there exists an affine contract maximizing the principal's worst-case objective. An affine contract is a linear contract with the addition of an ``offset" parameter. We use $\phi\in \bbR^{d+1}$ to represent an affine contract, and under this contract, the agent's payment function is $\phi(x) = \phi_0 + \sum_{i=1}^d \phi_i x_i$. First note that under an affine contract, the agent's best response will be the same for any compatible distribution, and hence yielding the principal the same payoff for any compatible distribution. 

% Now, given a non-affine contract $w(\cdot)$, we shall find an affine contract $\phi$ and a compatible distribution family $\cF$, such that the payoff of $\phi$ to the principal is no less than the payoff of $w(\cdot)$ under the compatible distribution family $\cF$. Then, since affine contracts yields the same payoff for any compatible distributions, this means $u(\phi) \ge u(w)$. Finally, given an affine contract $\phi$, we show that there must exists a linear contract $\phi$ which strictly improves upon the affine contract. Showing these completes the proof. 

% To proceed, we will find an affine contract $\phi$ whose payments are no less than those of $w$ for each possible outcome, in other words, $\phi$ is going to bound the function $w$ from above. To do so, we find all upper supporting hyperplanes for the lifted space $S = \set{ (x, w(x)) }$. Each of the upper supporting hyperplanes $H$ corresponds to a possible affine contract $\phi(H)$ which bounds $w$ from above. Now, for any action $a$ that the agent can take, he receives a no greater payment under $w$ than under $\phi(H)$. 

% So how to show existence of this hyperplane $H$? If we want the action $a(H)$ to have the same payment under $\alpha(H)$ and under $w$, then it suffices for the distribution of action $a(H)$ to only lie on the support of the hyperplane $H$ that touches the set $S = (x, w(x))$. In other words, it suffices for $a(H)$ to lie inside the convex hull of the support of $H$ (after projecting back to the ``unlifted set" $\mathcal{X}$. )

% Our next goal is to show that there exists some hyperplane $H$, with associated affine contract $\phi(H)$, and some specific compatible distributions $\cF$, such that for the incentivized action $a$ under $\phi(H)$, taking action $a$ gives the agent the same payment under $\phi(H)$ and under $w$. Hence, $\phi(H)$ and $w$ must incentivize the same action $a$ under this specific distribution $\cF$. From this, we know that the affine contract $\alpha(H)$ does no less than $w$ in the worst case. 



% Let us elaborate on the existence of such an affine contract and compatible distribution. For each possible upper supporting hyperplane $H$, let us consider the set of points on the support of $H$ and project these points back to $\mathcal{X}$, call this set $P(H)$. By a classic result in convex geometry, the union of the convex hulls of $P(H)$ over all $H$ is exactly the possible signal space $\mathcal{X}$. In other words, for each point $a\in \mathcal{A}$, there exists some hyperplane $H$ such that $a$ belongs to the convex hull of $P(H)$. Consider the function $g:\mathcal{H}\rightarrow \mathcal{H}$ which map a hyperplane $H$ to another hyperplane $H'$, such that the induced action $a$ under the affine contract associated with $H$ must belong to the convex hull of $P(H')$. Then, by a fixed-point theorem, there must exist some hyperplane $H$, such that the incentivized action under the affine contract associated with $H$ must lie within the convex hull of itself, $P(H)$. This precisely shows that we can let the compatible distribution be such that the action $a$ is only supported on the points in $P(H)$, and hence the payment for taking action $a$ remains the same under the affine contract and under $w$. 



% As the last step, we should that if the affine contract induces some action $a^*$, then there must exist a linear contract induces $a^*$ with a no greater payment to the agent. This finishes the proof. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%   END
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\textwidth]{media/plot_robust_new.png}
%     \caption{Illustration of the lifted set. The lifted set loosely resembles a square being foled slightly along the diagonal}
%     \label{fig:vis_robust}
% \end{figure}



% Once such a self-owned hyperplane \(H\) is identified, one can construct a compatible distribution whose support is contained in
% \[
% P(H)=\{x\in \mathcal{X} \mid (x,w(x))\in H\}.
% \]

% On these points, the affine contract \(\phi(H)\) and the original contract \(w\) yield the same payments. Moreover, since \(\phi(H)\) upper bounds \(w\) over all outcomes, any deviation yields no higher payment. Therefore, for this compatible distribution, the affine contract induces the same action as \(w\) with no greater payment, demonstrating that the affine contract performs at least as well as the original non-affine contract.

% This example captures the essence of our general proof: starting from any non-affine contract, one can employ the geometry of the lifted space and the notion of self-owned hyperplanes to construct an affine (and, ultimately, a linear) contract that is optimal for the principal’s worst-case objective. 



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Remove my old example
%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{An Example OLD}
% Before giving the proof to the theorem, we walkthrough a concrete example illustrating the proof idea. We start with a specific non-affine contract and show how to turn it into an affine contract, such that the affine contract performs no worse than the non-affine contract for some distribution. 

% Consider a setting with $d=2$ with a non-affine and non-linear contract $w$ as specified below. 
% \[
% w(0,0) = 0, w(1,0) = 2, w(0,1) = 2, w(1,1) = 3. 
% \]
% We can ``lift" the space $\mathcal{X} = \set{0,1}^2$ into $\bbR^3$ by appending the value of $w(x)$ as the last coordinate. In other words, the lifted space is the polytope defined by
% \[
% S = \set{ (0,0,0), (1,0,2), (0,1,2), (1,1,3) }. 
% \]
% If the contract were affine, the lifted polytope would just be a hyperplane. But of course the contract $w$ is not affine. There are two upper facets of $S$, each of which defines a hyperplane that bounds $S$ from above, the corresponding affine contracts are
% \[
% w(0,0) = 0, w(1,0) = 2, w(0,1) = 2, w(1,1) = 4,
% \]
% which is supported on the three points $X_1 = \{(0,0), (1,0), (0,1) \}$ in $\cX$. 
% and
% \[
% w(0,0) = 1, w(1,0) = 2, w(0,1) = 2, w(1,1) = 3, 
% \]
% which is supported on the three points $X_2 = \{(1,0), (0,1), (1,1) \}$ in $\cX$. 
% The interpolation between the two hyperplanes are also valid hyperplanes; these hyperplanes are supported on the two endpoints $(1,0)$ and $(0,1)$. 

% We claim that there must exist some hyperplane such that the induced action belongs to it's own support points after being projected back to $\cX$; call such a hyperplane ``self-owned". Suppose not, then the affine contract $w_1$ induces some action in $X_2$, and the affine contract $w_2$ induces some action in $X_1$. At the same time, the induced action is continuous in the sense that if we perturb the affine contract slightly, the induced action should not change much. Hence, as we continuously interpolate between $w_1$ and $w_2$, somewhere the induced action must fall exactly into the interval defined by $(1,0)$ and $(0,1)$, and hence we always have a ``self-owned" hyperplane. 

% Once we have such a ``self-owned" hyperplane $H$, we can construct compatible distributions where the support of the action $a$ is supported only on the support of $H$. On these points, the payment of the affine contract shares exactly the same payments as the original non-affine contract $w$. Further, since the affine contract bounds $w$ from above, any action receives a no greater payment. As such the affine contract induces the same action with no greater payment, and is no worse off then $w$ for this distribution. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% END Example OLD
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Then, by applying a fixed-point theorem, we can show that there must exists a hyperplane $H$ under which the incentivized action under the affine contract lies inside the support of the hyperplane $H$. Then, we can corresponding construct a distribution associated with the incentives action $a^*$, such that $a$ is only supported on the support of $H$, hence the payment for taking action $a^*$ remains the same under $w$ and under the affine contract defined by the hyperplane $H$. Further, since $H$ bounds $w$ from above, any action receives a no greater payment. Hence, action $a^*$ is incentives under the affine contract and at the same payment. 



% We will argue that for a carefully chosen distribution family, the incentivized action under $\phi$ is the same as the incentized action under contract $w()$. Note that for each action $a$, the agent receives a no greater payment under $w$ than under $\phi$. Moreover, we can carefully construct some distribution so that the payment of action $a^*$ is the same under the two contracts. suppose that the incentived action under $\phi$ is $a^*$, then we construct a compatible distribution $\cF$ and make it so that in the compatible distribution, the action $a^*$ is only supported on unchanged outcomes, i.e., for outcomes $x$ which $\phi(x) = w(x)$. Hence, the payment of $a^*$ remain unchanged. Then, the affine contract also incentivizes $a^*$ with the same payment, and must perform no worse than the contract $w(\cdot)$. 

% We now describe how one can construct such an affine contract. Recall the set of outcomes is $\mathcal{X} = [0,1]^d$, and that $w(\cdot)$ is a mapping from each possible outcome to a payment. We perform the so-called lifting operation and obtain a set of points in the $\bbR^{d+1}$ space:

% \[
% \set{ x\in\mathcal{X} : (x, w(x)) }. 
% \]

% Considering the set of facets on the lower convex hull of the set of points, if we project the facet back to the outcome space, they form a partition of the outcome space $\mathcal{X}$. Let the partition be $\set{ S_1, \dots, S_m }$, where each $S_i$ is a set of points in the original outcome space $\set{0,1}^d$, so that $\cup conv(S_j) = [0,1]^d$. 



% Now suppose we have obtained this partition (or triangulation). Each set $S_j$ corresponds to a lower facet in the lifted space, and represents a possible way to modify the contract: we can define the affine contract as being the hyperplane defined by this facet. Note that given a triangulation, only vertices that are outside the triangulation have their values decreased. The final step is then to show that there exists a lower facet, such that the incentivized action, call it $a^*$, under the modified contract as defined by $S_j$ must belong to the convex hull of $S_j$. Then, we can construct a compatible distribution such that $a^*$ is only supported on the points in $S_j$, and hence the payment to the agent if he should take $a^*$ remains unchanged. Therefore, recall that since $\phi < w$, the payment for any action does not increase and the payment for action $a^*$ is the same, $a^*$ is still incentivized under the affine contract. Hence the principal's under the affine contract $\phi$ must be no less than that under $w$. 




\fi
